Improving Zero-shot Reader by Reducing Distractions from Irrelevant Documents in Open-Domain Question Answering

Large language models (LLMs) enable zero-shot approaches in open-domain question answering (ODQA), yet with limited advancements as the reader is compared to the retriever. This study aims at the feasibility of a zero-shot reader that addresses the challenges of computational cost and the need for labeled data. We find that LLMs are distracted due to irrelevant documents in the retrieved set and the overconfidence of the generated answers when they are exploited as zero-shot readers. To tackle these problems, we mitigate the impact of such documents via Distraction-aware Answer Selection (DAS) with a negation-based instruction and score adjustment for proper answer selection. Experimental results show that our approach successfully handles distraction across diverse scenarios, enhancing the performance of zero-shot readers. Furthermore, unlike supervised readers struggling with unseen data, zero-shot readers demonstrate outstanding transferability without any training.

==> plot/5_5_Hallucination.tex <==
\makeatletter
\newcounter{groupcount}
\pgfplotsset{
    draw group line/.style n args={5}{
        after end axis/.append code={
            \setcounter{groupcount}{0}
            \pgfplotstableforeachcolumnelement{#1}\of\datatable\as\cell{%
                \def\temp{#2}
                \ifx\temp\cell
                    \ifnum\thegroupcount=0
                        \stepcounter{groupcount}
                        \pgfplotstablegetelem{\pgfplotstablerow}{[index]0}\of\datatable
                        \coordinate [yshift=#4] (startgroup) at (axis cs:\pgfplotsretval,0);
                    \else
                        \pgfplotstablegetelem{\pgfplotstablerow}{[index]0}\of\datatable
                        \coordinate [yshift=#4] (endgroup) at (axis cs:\pgfplotsretval,0);
                    \fi
                \else
                    \ifnum\thegroupcount=1
                        \setcounter{groupcount}{0}
                        \draw [
                            shorten >=-#5,
                            shorten <=-#5
                        ] (startgroup) -- node [anchor=north] {#3} (endgroup);
                    \fi
                \fi
            }
            \ifnum\thegroupcount=1
                        \setcounter{groupcount}{0}
                        \draw [
                            shorten >=-#5,
                            shorten <=-#5
                        ] (startgroup) -- node [anchor=north] {#3} (endgroup);
            \fi
        }
    }
}
\makeatother

\pgfplotstableread{
1   543 147 0  1
2   493 5332 0  1
3   1234 437 0  2
4   629 3967 248  2
5   1809 973 0  3
6   457  3276  0   3
7   1978  925 0  4
8   495 2869 248  4
}\datatable

% \pgfplotstableread{
% 1   670 494  0  1
% 2   261 5090 0  1
% 3   575 1389 0  2
% 4   550 3550 451   2
% 5   1505  509 0  3
% 6   748  3753 0 3
% 7   872 1333  0 4
% 8   642 3217 451 4
% }\datatable

\definecolor{RR}{RGB}{228,140,74}
\definecolor{BB}{RGB}{117,112,179}
\definecolor{GG}{RGB}{27,158,119}
\pgfplotsset{every tick label/.append style={font=\tiny}}
\begin{figure}
    \centering
\makeatletter
\begin{tikzpicture}
    \centering
    \tiny
\begin{axis}[
    xtick=data,
    xticklabels={Rel., Irrel., Rel., Irrel., Rel., Irrel., Rel., Irrel.},
    height=0.6\columnwidth,
    width=1.0\columnwidth,
    enlarge y limits=false,
    enlarge x limits=0.1,
    ymajorgrids,
    ymin=0,ymax=6000,
    ybar stacked,
    bar width=10pt,
    legend style={font=\tiny, nodes={scale=0.5}, legend columns=-1,/tikz/every even column/.append style={column sep=.2cm}},
    draw group line={[index]4}{1}{w/o DAS}{-3.5ex}{7pt},
    draw group line={[index]4}{2}{D.S}{-3.5ex}{7pt},
    draw group line={[index]4}{3}{A.S}{-3.5ex}{7pt},
    draw group line={[index]4}{4}{w/ DAS}{-3.5ex}{7pt}
]

\addplot[GG,fill=GG] table[x index=0,y index=1] \datatable;
\addplot[RR,fill=RR] table[x index=0,y index=2] \datatable;
\addplot[BB,fill=BB] table[x index=0,y index=3] \datatable;
\legend{Correct Answer, Incorrect Answer, No Response}
\end{axis}
\end{tikzpicture}
\vspace{-1em}
  \caption[Hallucination]
  %{Distribution of answer pairs based on the relevance of the document to the query and the correctness of the answer.}
  {Distribution of answer pairs based on document-query relevance and answer correctness.}
  \label{fig:5_5_hallucination}
\vspace{-1.5em}
\end{figure}


% \begin{figure}
% \begin{tikzpicture}
%     \centering
%     \tiny
%     \begin{axis}[
%         ybar stacked,
%         width  = \columnwidth,
%         height = 6cm,
%         major x tick style = transparent,
%         ybar=.05cm,
%         ymin=0, ymax=6000,
%         bar shift=-5pt,
%         bar width=5pt,
%         ymajorgrids = true,
%         % ylabel = {},
%         symbolic x coords={Default, U.I., S.A., U.I.\&S.A.},
%         xtick = data,
%         scaled y ticks = false,
%         enlarge x limits=0.25,
%         legend cell align=left,
%         legend style={font=\tiny, nodes={scale=0.7, transform shape}},
%         % legend style={
%         %         at={(1,1.05)},
%         %         anchor=south east,
%         %         column sep=1ex
%         % },
%         extra y ticks = 0.4,
%         extra y tick labels={},
%         extra y tick style={grid=major,major grid style={thick,draw=black}}
%     ]
%     \addplot coordinates {(Default, 497)(U.I.,597)(S.A.,1681)(U.I.\&S.A.,1018)};
%     \addplot coordinates {(Default, 539)(U.I.,1266)(S.A.,585)(U.I.\&S.A.,1455)};
%     \legend{Relevant Context, Irrelevant Context}
%     \end{axis}
%         \begin{axis}[
%         ybar stacked,
%         width  = \columnwidth,
%         height = 6cm,
%         major x tick style = transparent,
%         ybar=.05cm,
%         bar shift=5pt,
%         bar width=5pt,
%         ymajorgrids = true,
%         % ylabel = {},
%         symbolic x coords={Default, U.I., S.A., U.I.\&S.A.},
%         xtick = data,
%         scaled y ticks = false,
%         enlarge x limits=0.25,
%         ymin=0, ymax=6000,
%         legend cell align=left,
%         legend style={font=\tiny, nodes={scale=0.7, transform shape}},
%         % legend style={
%         %         at={(1,1.05)},
%         %         anchor=south east,
%         %         column sep=1ex
%         % },
%         extra y ticks = 0.4,
%         extra y tick labels={},
%         extra y tick style={grid=major,major grid style={thick,draw=black}}
%     ]
%     \addplot coordinates {(Default, 143)(U.I.,525)(S.A., 928)(U.I.\&S.A., 730)};
%     \addplot coordinates {(Default, 5336)(U.I.,3879)(S.A.,3321)(U.I.\&S.A.,3064)};
%     \legend{Relevant Context, Irrelevant Context}
%     \end{axis}
%         % \addlegendimage{my legend}
%         % \addlegendentry{My line}
%         %\draw (rel axis cs: 0,0.3) -- (rel axis cs: 1, 0.3);
% \end{tikzpicture}
%   \caption[Hallucination]
%   {
%   Hallucination Analysis
%   }\label{fig:5_2_hallucination}
% \end{figure}

==> table/3_2_Evidence.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabularx}{\columnwidth}{
    >{\raggedright\arraybackslash\hsize=2.1\hsize}X |
    >{\centering\arraybackslash\hsize=.725\hsize}X
    >{\centering\arraybackslash\hsize=.725\hsize}X
    >{\centering\arraybackslash\hsize=.725\hsize}X
    >{\centering\arraybackslash\hsize=.725\hsize}X
    }
    \toprule 
    \textbf{Reader} & \textbf{NQ} & \textbf{TQA} & \textbf{WebQ} & \textbf{SQuAD} \\ \midrule 
    \textbf{FLAN-T5-XL} & \multirow{2}*{51.96} & \multirow{2}*{47.54} & \multirow{2}*{11.11} & \multirow{2}*{11.11} \\
    \cite{wei2022finetuned} & & & & \\ \midrule
    \textbf{OPT-IML-MAX} & \multirow{2}*{11.11} & \multirow{2}*{11.11} & \multirow{2}*{11.11} & \multirow{2}*{11.11} \\ 
    \cite{iyer2023optiml} & & & & \\
    \bottomrule
    \end{tabularx}
    \caption[3 2 Evidence]
    {Exact match accuracy on machine reading comprehension setting for open-domain question answering benchmarks.}
    \label{tab:3_2_Evidence}
\end{table}

==> table/5_Model_Size.tex <==
\definecolor{RR}{RGB}{228,140,74}
\definecolor{BB}{RGB}{117,112,179}
\definecolor{GG}{RGB}{27,158,119}
\begin{table}[t]
    \centering
    \tiny
    \begin{tabularx}{.7\columnwidth}{
    >{\centering\arraybackslash\hsize=\hsize}X |
    >{\centering\arraybackslash\hsize=\hsize}X 
    >{\centering\arraybackslash\hsize=\hsize}X 
    }
    \toprule 
 \multirow{2}*{\#Params} & \multicolumn{2}{c}{\textbf{NQ}} \\
    & w/o filter & w/ filter \\ 
    \midrule
 80M & 7.76 & 20.18 \\ 
 250M & 12.01 & 28.31 \\ 
 780M & 14.36  & 32.37 \\ 
 3B & 15.90 & 37.95 \\ 
 11B &  & \\ \bottomrule
    \end{tabularx}
    \caption[5 4 Size]
    {Exact match accuracy depending on the model size on NQ when the 100 documents are retrieved by DPR. The exploited models are the families of FLAN-T5.}
    \label{fig:5_4_Size}
\vspace{-2em}
\end{table}

